High-Fidelity Polarization Storage in a Gigahertz Bandwidth Quantum Memory

We demonstrate a dual-rail optical Raman memory inside a polarization interferometer; this enables us to store polarization-encoded information at GHz bandwidths in a room-temperature atomic ensemble. By performing full process tomography on the system we measure up to 97\pm1% process fidelity for the storage and retrieval process. At longer storage times, the process fidelity remains high, despite a loss of efficiency. The fidelity is 86\pm4% for 1.5 \mu s storage time, which is 5,000 times the pulse duration. Hence high fidelity is combined with a large time-bandwidth product. This high performance, with an experimentally simple setup, demonstrates the suitability of the Raman memory for integration into large-scale quantum networks.

==> preamble.tex <==
\usepackage{color}
\usepackage{epstopdf}
\usepackage{fancyhdr}
\usepackage[square, sort&compress, super, comma, numbers]{natbib}
\usepackage{amsmath}
\usepackage[a4paper, textwidth=14cm, textheight=21cm, centering, headsep=1cm]{geometry}
\usepackage{setspace}
\usepackage[labelsep=quad, font={small}, labelfont=bf, width=0.75\textwidth, aboveskip=1cm, belowskip=0cm]{caption}
\usepackage{sectsty}
\usepackage{rotating}
\usepackage{abbrevs}
\usepackage{graphicx,xspace}
\usepackage{units}
\usepackage{hyperref}
%\hypersetup{
%colorlinks=false,
%linkbordercolor={1 1 1}, % set to white
%citebordercolor={0 0 0} % set to white
%} 
\usepackage{color,hyperref}
\definecolor{darkblue}{rgb}{0.0,0.0,0}
\hypersetup{colorlinks,breaklinks,
        linkcolor=darkblue,urlcolor=darkblue,
           anchorcolor=darkblue,citecolor=darkblue}
%\usepackage[hyperpageref]{backref}





%\doublespace
\setstretch{1}

%\setlength{\footnotesep}{\baselinestretch\footnotesep}

\newcommand{\mycomment}[1]{\textbf{\textcolor{red}{#1}}}
\newcommand{\bra}[1]{\langle #1 |}
\newcommand{\ket}[1]{| #1 \rangle}
\newcommand{\braket}[2]{\langle #1 | #2 \rangle}
\newcommand{\expectation}[1]{\langle #1 \rangle}
\newcommand{\creatop}[1]{\hat{a}^{\dagger}_{#1}}
\newcommand{\anniop}[1]{\hat{a}_{#1}}

%Centre chapter headings
\chapterfont{\centering}

% Set page style for main document

\pagestyle{fancy}
%\renewcommand{\chaptermark}[1]{\markboth{\MakeUppercase{\thechapter. #1 }}{}}
%\renewcommand{\sectionmark}[1]{\markright{\thesection\ #1}}
\renewcommand{\sectionmark}[1]{\markright{\thesection\ #1}}
\fancyhf{}
\fancyhead[RO]{\bfseries\rightmark}
\fancyhead[LE]{\bfseries\leftmark}
\fancyfoot[C]{\thepage}
\fancyhead[R]{Engl1202}
\fancyhead[L]{\bfseries\title}
\renewcommand{\headrulewidth}{0pt}
\renewcommand{\footrulewidth}{0.5pt}
\addtolength{\headheight}{0.5pt}
\fancypagestyle{plain}{
\fancyhead{}
\renewcommand{\headrulewidth}{0pt}}



% Set environment parameters for dedication, abstract, and acknowledgements


